Continuous-Time Reinforcement Learning: New Design Algorithms with Theoretical Insights and Performance Guarantees

Continuous-time nonlinear optimal control problems hold great promise in real-world applications. After decades of development, reinforcement learning (RL) has achieved some of the greatest successes as a general nonlinear control design method. However, a recent comprehensive analysis of state-of-the-art continuous-time RL (CT-RL) methods, namely, adaptive dynamic programming (ADP)-based CT-RL algorithms, reveals they face significant design challenges due to their complexity, numerical conditioning, and dimensional scaling issues. Despite advanced theoretical results, existing ADP CT-RL synthesis methods are inadequate in solving even small, academic problems. The goal of this work is thus to introduce a suite of new CT-RL algorithms for control of affine nonlinear systems. Our design approach relies on two important factors. First, our methods are applicable to physical systems that can be partitioned into smaller subproblems. This constructive consideration results in reduced dimensionality and greatly improved intuitiveness of design. Second, we introduce a new excitation framework to improve persistence of excitation (PE) and numerical conditioning performance via classical input/output insights. Such a design-centric approach is the first of its kind in the ADP CT-RL community. In this paper, we progressively introduce a suite of (decentralized) excitable integral reinforcement learning (EIRL) algorithms. We provide convergence and closed-loop stability guarantees, and we demonstrate these guarantees on a significant application problem of controlling an unstable, nonminimum phase hypersonic vehicle (HSV).

==> bios.tex <==
% ************************************************************************
% ************************************************************************
% ************************************************************************
%
% BIOS
%
% ************************************************************************
% ************************************************************************
% ************************************************************************

% ************************************************************************
% ************************************************************************
%
% BIO -- B. A. Wallace
%
% ************************************************************************
% ************************************************************************

Brent Wallace received his B.S. degree from Arizona State University, Tempe, AZ, USA in 2019. Currently, he is pursuing his Ph.D. with the Department of Electrical, Computer \& Energy Engineering, Arizona State University, Tempe, AZ, USA. 

He was a Research Intern with The Aerospace Corporation Microelectronics Group, El Segundo, CA, USA. His current interests include adaptive dynamic programming, nonlinear optimal control, and control applications in aerospace systems. 

Brent Wallace received National Science Foundation (NSF) Graduate Research Fellowship in 2020.

% ************************************************************************
% ************************************************************************
%
% BIO -- J. Si
%
% ************************************************************************
% ************************************************************************
